Information flows in nanomachines

Nanomachines are often interpreted as autonomous Maxwell's demons or information engines. This interpretation is appealing from a conceptual viewpoint but sometimes lacks a rigorous and precise formulation. Moreover, it is unclear whether this interpretation is truly useful for analyzing the performance of nanomachines or designing more efficient ones. The concepts of mutual information and information flows provide a quantitative and rigorous account of the role of information in physical systems. In this chapter, we present a pedagogical review of these concepts and apply them to a specific energy transducer at the nanoscale, which couples the tunnel transport of electrons through a carbon nanotube with its mechanical oscillations.

==> driven_case.tex <==
\subsection{Driven case}
\label{sec:nonautCNT}


Now, we will examine the device's performance in terms of information flows. Let's start by considering the driven scenario, where the nanotube is externally excited by a radio-frequency pulse with a frequency of $\Omega$. This pulse triggers the oscillations of the carbon nanotube. In Figure \ref{fig:non_autonomous} (top, red curve), you can observe the average position of the oscillator $\langle x\rangle$ over a single time period of $2\pi / \Omega$. In this figure, $\varphi \in [0, 2\pi]$ represents the instantaneous phase of the driving pulse.

For positive bias voltage $V_{SD} > 0$, the average electron occupation follows a periodic evolution synchronized with the oscillation, as shown in Figure \ref{fig:non_autonomous} (top, blue line). As the nanotube moves upwards $\varphi \simeq \pi$, the quantum dot is pushed above the chemical potentials $\mu_{S,D}$ and becomes empty. As the nanotube descends again $\varphi\simeq 0,2\pi$, the dot refills.
\begin{figure}
    \centering    \includegraphics[width = 0.9\linewidth]{phase_evolution.pdf}
    \caption{Non-autonomous implementation of the device. \textit{Top left}: Average position (red) and occupation (blue) of the system along the oscillations in terms of the stroboscopic phase $\varphi$. \textit{Bottom left}: Mutual information (green) and information flows $\dot I_{\rm osc}$ (red) and $\dot I_{\rm dot}$ (blue) along the oscillation. \textit{Top right}: Shannon entropy of the quantum dot $S_{\rm dot}$ and time derivative $\dot S_{\rm dot}$. \textit{Bottom right}: heat flow in the dot $\dot Q_{\rm dot}$. $\tau = 2\pi/\Omega$ is the oscillation period. $\Omega/(2\pi)=270$ MHz, $g=0.01$~eV$/$nm, $m =2\times 10^{-22}$ kg, and $Q = 1000$. $V_{SD} = 1$ eV and $T = T_S = T_D = 40$mK and $k = 1$. We also consider homogeneous tunnel barriers, $\alpha_\mathrm{ S,D} = 0$ and $\gamma_\mathrm{ S,D} = 100\Omega$. In this configuration, the dot switches between a state with average occupation $\langle p\rangle = 0.5$ and $\langle p\rangle = 0$ each time the oscillator moves through $x=0$.}
    \label{fig:non_autonomous}
\end{figure}

It is worth noting that in this scenario, the time-dependent driving acting on the system implies a time-dependent density function $\rho(x,v,p;t)$, therefore $\dot I \neq 0$ and $\dot S_{\rm dot} \neq 0$. In Fig.\ref{fig:non_autonomous}(top right) we represent $\dot S_{\rm dot}$ as a function of the phase $\varphi$. As one can observe, the Shannon entropy of the quantum dot changes abruptly near the points $\varphi = \pi/2$ and $\varphi = 3\pi/2$, where the average occupation changes from $\langle p \rangle = 1/2$ to 0 and \textit{vice versa}. The state with $\langle p \rangle = 1/2$ represents the maximal entropy state, while the state with $\langle p \rangle = 0$ has no entropy.

The entropy changes are associated with two peaks of mutual information $I(x,v;p)$, plotted in Fig.\ref{fig:non_autonomous} (bottom left). At these peaks, the oscillator

Remarkably, the information flows, shown in Figure \ref{fig:non_autonomous} (bottom, red and blue lines), also reach maximum values during these occupation changes, with their sign reversing at each peak. Around $\varphi \sim \pi/2$, $\dot I^{\rm dot} > 0$, indicating that the quantum dot functions as a demon in accordance with the discussion under Eq.\eqref{secondflows}. Similarly, at $\varphi \sim 3\pi/2$, $\dot I^{\rm osc} > 0$, implying that the oscillator itself acts as a demon.

For deeper insights into the thermodynamics of the driven case, we can shift our focus to the quantum dot occupation and consider Eq.\eqref{seclawdot}. Integrating the inequality on time from $\varphi = 0$ to $\varphi = \pi$ we obtain
\begin{equation}
    -k\log 2 - \Delta I^{\rm dot} -\frac{Q_{\rm er}}{T}\geq 0.
\end{equation}
Here, the term $-k\log 2$ represents the change in Shannon entropy when the quantum dot average occupation transitions from $\langle p \rangle = 1/2$ to 0. Meanwhile, the term $-Q_{\rm er}/T$ represents the entropy released into the environment through heat exchange, denoted as $Q_{\rm er} < 0$. Here, $\Delta I^{\rm dot}$ signifies the integrated information flow during this process. As depicted in Figure \ref{fig:non_autonomous}, $\Delta I^{\rm dot} > 0$.

From an informational perspective, when the nanotube moves upwards, the quantum dot's occupation resets from a mixed state of 0 and 1 to a definite state of 0, resulting in a reduction of its Shannon information. This phenomenon is termed \textit{Landauer's erasure} \cite{Landauer1961, Elouard_2015}. As indicated by the preceding inequality, this process necessitates a minimal energy dissipation of $kT\log 2 + T\Delta I^{\rm dot} > 0$ into the environment. Notably, the presence of information flow amplifies the energy requirement for this operation.

Conversely, the inverse process takes place from $\varphi = \pi$ to $\varphi = 2\pi$. Within this interval, the quantum dot's state shifts from an occupation of 0 to a mixed state encompassing 0 and 1, leading to an augmentation in the entropy of the quantum dot.
 
Integrating Eq.\eqref{seclawdot} along this process we obtain 
\begin{equation}
    k\log 2 - \Delta I^{\rm dot} -\frac{Q_{\rm mot}}{T}\geq 0.
    \label{eq:motor}
\end{equation}
In this inequation $Q_{\rm mot}$ represents the heat exchanged with the environment along this process, and according to Fig.\ref{fig:non_autonomous}, $\Delta I^{\rm dot} < 0$.

The latter process bears similarity to the expansion observed in the Szilárd engine, illustrated in Figure \ref{fig:szilard}, subsequent to the measurement of particle position. In that scenario, the system exploits the entropy alteration in the quantum dot to draw a specific energy $Q_{\rm mot} > 0$ from the environment, effectively functioning as a motor. Leveraging the preceding outcome, we ascertain that the maximum retrievable heat for the nanotube in this operation amounts to $\log 2 - \Delta I^{\rm dot}\geq 0$. Notably, in this case, the information flow curtails the efficiency of the motor.

==> latexmkrc <==
$makeindex  = 'makeindex -s svind.ist %O -o %D %S';

$ENV{'TEXINPUTS'}='./style//:' . $ENV{'TEXINPUTS'}; 
$ENV{'BSTINPUTS'}='./style//:' . $ENV{'BSTINPUTS'}; 

###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for Overleaf v2
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    my $QPDF = "/usr/bin/qpdf";
    return if ! -x $QPDF; # check that qpdf exists
    my $status = system($QPDF, "--linearize", "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
	system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
        $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
	system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
	if (-e $rtex_file) {
		do_knitr($rtex_file);
	}
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
	# change directory for a limited scope
	my $orig_dir = cwd();
	my $subdir = dirname($target);
	chdir($subdir);
	# run chktex on main file
	$status = system(
    "/usr/bin/run-chktex.sh",
    $orig_dir,
    $file
  );
	# go back to original directory
	chdir($orig_dir);

	# in VALIDATE mode we always exit after running chktex
	# otherwise we exit if EXIT_ON_ERROR is set

	if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
	    # chktex doesn't let us access the error info via exit status
	    # so look through the output
	    open(my $fh, "<", "output.chktex");
	    my $errors = 0;
	    {
		local $/ = "\n";
		while(<$fh>) {
		    if (/^\S+:\d+:\d+: Error:/) {
			$errors++;
			print;
		    }
		}
	    }
	    close($fh);
	    exit(1) if $errors > 0;
	    exit(0) if $ENV{'CHKTEX_VALIDATE'};
	}
    }
}


==> style/references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} If the citatiion in the text is numbered, the reference list should be arranged in ascending order. If the citation in the text is author/year, the reference list should be \textit{sorted} alphabetically and if there are several works by the same author, the following order should be used:
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer Nature style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
\bigskip
%
% Journal article
\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O'Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}

